Child Care, Time Allocation, and the Life Cycle

This study explores the impact of gender differences in preferences and productivity in home production on the time allocation in married couples, particularly in relation to childcare responsibilities. Using aggregated data from Japan, we estimate a life-cycle model that tracks the development of a child from infancy to adulthood by extending the work of Blundell et al. (2018). Our findings reveal a decrease in maternal earnings following childbirth, aligning with the empirical evidence of the child penalty. However, the model's projections and the actual data diverge significantly during the phase of maternal earnings recovery, showing a discrepancy of approximately 50%, the size of which implies an involuntary reduction in the wife's market work earnings.

==> Tables/table_2_parameters_est_market_house_work.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tb]
\caption{Estimation of Parameters}
\label{tab:parameters}
\begin{center}

\begin{footnotesize}
(a) MRS Parameters


\begin{tabular}{c|c|c|c|c|c}
\hline 
%\multirow{}{}{} & \multicolumn{5}{c|}{MRS parameters}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 \multicolumn{3}{c|}{Leisure and Consumption} &   \multicolumn{3}{c}{Parental Time}\tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Our Estimation & Blundell et al (2018) &  & Our Estimation & Blundell et al (2018)\tabularnewline
 \hline
$\psi_{L1}$ & 0.1970 & 0.211 & $\psi_{T1}$ & 0.2023 & 0.115\tabularnewline
 
$\psi_{L2}$ & 0.1444 & 0.162 & $\psi_{T2}$ & 0.5703 & 0.503\tabularnewline
 
$\rho_{L}$ & 0.4830 & 0.535 & $\rho_{T}$ & -0.1733 & -0.197\tabularnewline
e 
$\eta$ & 0.5083 & 0.903 &  &  & \tabularnewline
\hline 
\end{tabular}

\bigskip{}

(b) Preference Shifters

\begin{tabular}{c|c|c|c|c}
\hline 
%\multirow{}{}{} & \multicolumn{4}{c|}{Preference Shifters}\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & \multicolumn{2}{c|}{With Children} & \multicolumn{2}{c}{Without Children}\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & Our Estimation & Blundell et al (2018) & Our Estimation & Blundell et al (2018)\tabularnewline
\hline 
$\Phi_{L1} (Age 20)$  & -8.5765 & -8.925 & -6.0536 & -7.680\tabularnewline
 
$\Phi_{L2} (Age 20)$ & -8.9871 & -9.397 & -8.9352 & -8.816\tabularnewline
 
$\Phi_{T1}(Age 30)$ & -20.7575 & -23.993 & na & na\tabularnewline
 
$\Phi{}_{T2}(Age 30)$ & -3.3493 & -3.957 & na & na\tabularnewline
 
$\Phi_{C}$ & -0.9656 & 0.132 & -1.0 (fixed) & 0 (fixed) \tabularnewline
\hline 
\end{tabular}


\end{footnotesize}
\end{center}


\vspace{0.5\baselineskip}
    \begin{footnotesize}
Note: (1) The preference for leisure time is set equal for husbands and wives of married couples, i.e., $\Phi_{L1} = \Phi_{L2}$. (2) Wives have more preferable choices for childcare time than leisure time, i.e., $\Phi_{T2} > \Phi_{L2}$. (3) And wives have a more extensive selection for child care than the husband, i.e., $\Phi_{T2} > \Phi_{T1}$.   (4) childcare preferences are assumed to be determined by the child's age, with a maximum at the child's age zero (or Parental age 30) and decreasing linearly until the child reaches age 18 as shown in Figure \ref{fig:time_varying_preference}
\end{footnotesize}

\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Tables/table_2_parameters_est_only_market_work.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tb]
\caption{Estimation of Parameters}
\label{tab:parameters}
\begin{center}

\begin{footnotesize}
(a) MRS parameters


\begin{tabular}{c|c|c|c|c|c}
\hline 
%\multirow{}{}{} & \multicolumn{5}{c|}{MRS parameters}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 \multicolumn{3}{c|}{Leisure and Consumption} &   \multicolumn{3}{c}{Parental Time}\tabularnewline
%\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & Our estimation & Blundell et al (2018) &  & Our estimation & Blundell et al (2018)\tabularnewline
 \hline
$\psi_{L1}$ & 0.2057 & 0.211 & $\psi_{T1}$ & 0.2020 & 0.115\tabularnewline
 
$\psi_{L2}$ & 0.1534 & 0.162 & $\psi_{T2}$ & 0.5023 & 0.503\tabularnewline
 
$\rho_{L}$ & 0.5173 & 0.535 & $\rho_{T}$ & -0.2006 & -0.197\tabularnewline
e 
$\eta$ & 0.5127 & 0.903 &  &  & \tabularnewline
\hline 
\end{tabular}

\bigskip{}

(b) Preference Shifters

\begin{tabular}{c|c|c|c|c}
\hline 
%\multirow{}{}{} & \multicolumn{4}{c|}{Preference Shifters}\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & \multicolumn{2}{c|}{With Children} & \multicolumn{2}{c}{without Children}\tabularnewline
%\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & Our estimation & Blundell et al (2018) & Our estimation & Blundell et al (2018)\tabularnewline
\hline 
$\Phi_{L1} (Age 20)$  & -9.0530 & -8.925 & -7.3446 & -7.680\tabularnewline
 
$\Phi_{L2} (Age 20)$ & -8.2593 & -9.397 & -6.7381 & -8.816\tabularnewline
 
$\Phi_{T1}(Age 30)$ & -20.1350 & -23.993 & na & na\tabularnewline
 
$\Phi{}_{T2}(Age 30)$ & -3.0030 & -3.957 & na & na\tabularnewline
 
$\Phi_{C}$ & -1.0122 & 0.132 & -1.0 (fixed) & 0 (fixed) \tabularnewline
\hline 
\end{tabular}


\end{footnotesize}
\end{center}


\vspace{0.5\baselineskip}
    \begin{footnotesize}
Note: (1) the preference for leisure time is set equal for husbands and wives of married couples, i.e., $\Phi_{L1} = \Phi_{L2}$. (2) Wives have more preferable choices for child care time than leisure time, i.e., $\Phi_{T2} > \Phi_{L2}$. (3) And wives have a more extensive selection for child care than the husband, i.e., $\Phi_{T2} > \Phi_{T1}$.   (4) childcare preferences are assumed to be determined by the child's age, with a maximum at the child's age zero (or Parental age 30) and decreasing linearly until the child reaches age 18 as shown in Figure \ref{fig:time_varying_preference}
\end{footnotesize}

\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Tables/table_parameters.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tb]
\caption{Parameter Setting}
\label{tab:parameters}
\begin{center}
\begin{small}
\begin{tabular}{|c|c|c|c|}
\hline 
 & \multicolumn{3}{c|}{(a) MRS parameters}\tabularnewline
\hline 
 & Leisure and Consumption &  & Parental Time\tabularnewline
\hline 
$\psi_{L1}$ & 0.2 (0.211) & $\psi_{T1}$ & 0.1 (0.115)\tabularnewline
\hline 
$\psi_{L2}$ & 0.15 (0.162) & $\psi_{T2}$ & 0.5 (0.503)\tabularnewline
\hline 
$\rho_{L}$ & 0.5 (0.535) & $\rho_{T}$ & $-0.2$ ($-0.197$)\tabularnewline
\hline 
$\eta$ & 0.5 (0.903) &  & \tabularnewline
\hline 

\end{tabular}

\bigskip{}

\begin{tabular}{|c|c|c|}
\hline 
 & \multicolumn{2}{c|}{(b) Preference Shifters}\tabularnewline
\hline 
 & With Children & without Children\tabularnewline
\hline 
$\Phi_{L1}$ $(Age=20)$ & $-8.5$ ($-8.925$) & $-7.0$ ($-7.680$)\tabularnewline
\hline 
$\Phi{}_{L2}$ $(Age=20)$ & $-8.5$ ($-9.397$) & $-8.0$ ($-8.816$)\tabularnewline
\hline 
$\Phi_{T1}$ $(KidAge=0)$ & $-20.0$ ($-23.993$) & na\tabularnewline
\hline 
$\Phi{}_{T2}$ $(KidAge=0)$ & $-3.0$ ($-3.957$) & na\tabularnewline
\hline 
$\Phi_{C}$ & $-1.0$ (0.132) & $-1.0$ (0)\tabularnewline
\hline 
\end{tabular}
\end{small}

\vspace{0.5\baselineskip}
    \begin{footnotesize}
    Note: The values in parentheses in  Table 1 are the estimates of \citet{blundellChildrenTimeAllocation2018}. 
    \end{footnotesize}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Tables/table_parameters_1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tb]
\caption{Parameter Setting}
\label{tab:parameters}
\begin{center}
(a) MRS parameters

\begin{footnotesize}
\begin{tabular}{|c|c|c|c|c|c|}
\hline 
%\multirow{}{}{} & \multicolumn{5}{c|}{MRS parameters}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & \multicolumn{2}{c|}{Leisure and Consumption} &  & \multicolumn{2}{c|}{Parental Time}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & calibration & Blundell et al (2018) &  & calibration & Blundell et al (2018)\tabularnewline
\hline 
$\psi_{L1}$ & 0.2 & 0.211 & $\psi_{T1}$ & 0.1 & 0.115\tabularnewline
\hline 
$\psi_{L2}$ & 0.15 & 0.162 & $\psi_{T2}$ & 0.5 & 0.503\tabularnewline
\hline 
$\rho_{L}$ & 0.5 & 0.535 & $\rho_{T}$ & -0.2 & -0.197\tabularnewline
\hline 
$\eta$ & 0.5 & 0.903 &  &  & \tabularnewline
\hline 
\end{tabular}

\bigskip{}

(b) Preference Shifters

\begin{tabular}{|c|c|c|c|c|}
\hline 
%\multirow{}{}{} & \multicolumn{4}{c|}{Preference Shifters}\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & \multicolumn{2}{c|}{With Children} & \multicolumn{2}{c|}{without Children}\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} 
 & calibration & Blundell et al (2018) & calibration & Blundell et al (2018)\tabularnewline
\hline 
$\Phi_{L1} (Age 20)$  & -8.5 & -8.925 & -7.0 & -7.680\tabularnewline
\hline 
$\Phi{}_{L2} (Age 20)$ & -8.5 & -9.397 & -8.0 & -8.816\tabularnewline
\hline 
$\Phi_{T1}(Age 30)$ & -20.0 & -23.993 & na & na\tabularnewline
\hline 
$\Phi{}_{T2}(Age 30)$ & -3.0 & -3.957 & na & na\tabularnewline
\hline 
$\Phi_{C}$ & -1.0 & 0.132 & -1.0 & 0\tabularnewline
\hline 
\end{tabular}


\end{footnotesize}
\end{center}


\vspace{0.5\baselineskip}
    \begin{footnotesize}
Note: (1) the preference for leisure time is set equal for husbands and wives of married couples, i.e., $\Phi_{L1} = \Phi_{L2}$. (2) Wives have more preferable choices for child care time than leisure time, i.e., $\Phi_{T2} > \Phi_{L2}$. (3) And wives have a more extensive selection for child care than the husband, i.e., $\Phi_{T2} > \Phi_{T1}$.   (4) childcare preferences are assumed to be determined by the child's age, with a maximum at the child's age zero (or Parental age 30) and decreasing linearly until the child reaches age 18 as shown in Figure \ref{fig:time_varying_preference}
\end{footnotesize}

\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
